Towards Hybrid Two-Phase Modelling Using Linear Domain Decomposition

The viscous flow of two immiscible fluids in a porous medium on the Darcy scale is governed by a system of nonlinear parabolic equations. If infinite mobility of one phase can be assumed (e.g. in soil layers in contact with the atmosphere) the system can be substituted by the scalar Richards model. Thus, the domain of the porous medium may be partitioned into disjoint subdomains with either the full two-phase or the simplified Richards model dynamics. Extending the one-model approach from [1, 2] we suggest coupling conditions for this hybrid model approach. Based on an Euler implicit discretisation, a linear iterative (-type) domain decomposition scheme is proposed, and proven to be convergent. The theoretical findings are verified by a comparative numerical study that in particular confirms the efficiency of the hybrid ansatz as compared to full two-phase model computations.

==> Praeamble_and_definitions/LDD_special_symbols.tex <==
%% SPECIAL INTEGRAL SIGNS
% The following example defines macro
% 
% \mint{<symbol>}\limits_{...} ^{...} %statt \limits kann auch  \nolimits \displaylimits_stehen
% 
%     The first argument is the symbol that is put in smaller math style in the middle of the integral symbol.
%     Then a limits specification follows, any number and order. The last one is used.
%     Then one subscript and/or one superscript can follow in any order, but at most one of each type.
% 
% The implementation takes care of:
% 
%     the current math style,
%     calculates the correct position for the middle of the integral
%     even, if subscript and/or superscript are given with \limits,
%     lets the horizontal spacing around the symbol intact and
%     is aware of \mathsurround.


\makeatletter
\newcommand*{\mint}[1]{%
  % #1: overlay symbol
  \mint@l{#1}{}%
}
\newcommand*{\mint@l}[2]{%
  % #1: overlay symbol
  % #2: limits
  \@ifnextchar\limits{%
    \mint@l{#1}%
  }{%
    \@ifnextchar\nolimits{%
      \mint@l{#1}%
    }{%
      \@ifnextchar\displaylimits{%
        \mint@l{#1}%
      }{%
        \mint@s{#2}{#1}%
      }%
    }%
  }%
}
\newcommand*{\mint@s}[2]{%
  % #1: limits
  % #2: overlay symbol
  \@ifnextchar_{%
    \mint@sub{#1}{#2}%
  }{%
    \@ifnextchar^{%
      \mint@sup{#1}{#2}%
    }{%
      \mint@{#1}{#2}{}{}%
    }%
  }%
}
\def\mint@sub#1#2_#3{%
  \@ifnextchar^{%
    \mint@sub@sup{#1}{#2}{#3}%
  }{%
    \mint@{#1}{#2}{#3}{}%
  }%
}
\def\mint@sup#1#2^#3{%
  \@ifnextchar_{%
    \mint@sub@sup{#1}{#2}{#3}%
  }{%
    \mint@{#1}{#2}{}{#3}%
  }%
}
\def\mint@sub@sup#1#2#3^#4{%
  \mint@{#1}{#2}{#3}{#4}%
}
\def\mint@sup@sub#1#2#3_#4{%
  \mint@{#1}{#2}{#4}{#3}%
}
\newcommand*{\mint@}[4]{%
  % #1: \limits, \nolimits, \displaylimits
  % #2: overlay symbol: -, =, ...
  % #3: subscript
  % #4: superscript
  \mathop{}%
  \mkern-\thinmuskip
  \mathchoice{%
    \mint@@{#1}{#2}{#3}{#4}%
        \displaystyle\textstyle\scriptstyle
  }{%
    \mint@@{#1}{#2}{#3}{#4}%
        \textstyle\scriptstyle\scriptstyle
  }{%
    \mint@@{#1}{#2}{#3}{#4}%
        \scriptstyle\scriptscriptstyle\scriptscriptstyle
  }{%
    \mint@@{#1}{#2}{#3}{#4}%
        \scriptscriptstyle\scriptscriptstyle\scriptscriptstyle
  }%
  \mkern-\thinmuskip
  \int#1%
  \ifx\\#3\\\else_{#3}\fi
  \ifx\\#4\\\else^{#4}\fi  
}
\newcommand*{\mint@@}[7]{%
  % #1: limits
  % #2: overlay symbol
  % #3: subscript
  % #4: superscript
  % #5: math style
  % #6: math style for overlay symbol
  % #7: math style for subscript/superscript
  \begingroup
    \sbox0{$#5\int\m@th$}%
    \sbox2{$#5\int_{}\m@th$}%
    \dimen2=\wd0 %
    % => \dimen2 = width of \int
    \let\mint@limits=#1\relax
    \ifx\mint@limits\relax
      \sbox4{$#5\int_{\kern1sp}^{\kern1sp}\m@th$}%
      \ifdim\wd4>\wd2 %
        \let\mint@limits=\nolimits
      \else
        \let\mint@limits=\limits
      \fi
    \fi
    \ifx\mint@limits\displaylimits
      \ifx#5\displaystyle
        \let\mint@limits=\limits
      \fi
    \fi
    \ifx\mint@limits\limits
      \sbox0{$#7#3\m@th$}%
      \sbox2{$#7#4\m@th$}%
      \ifdim\wd0>\dimen2 %
        \dimen2=\wd0 %
      \fi
      \ifdim\wd2>\dimen2 %
        \dimen2=\wd2 %
      \fi
    \fi
    \rlap{%
      $#5%
        \vcenter{%
          \hbox to\dimen2{%
            \hss
            $#6{#2}\m@th$%
            \hss
          }%
        }%
      $%
    }%
  \endgroup
}
% EXAMPLE INTEGRAL SIGNS
% \begin{document}
% \[
%   \displaystyle A\int B
%   \textstyle A\int B
%   \scriptstyle A\int B
%   \scriptscriptstyle A\int B
% \]
% \[
%   \displaystyle A\mint{-} B
%   \textstyle A\mint{-} B
%   \scriptstyle A\mint{-} B
%   \scriptscriptstyle A\mint{-} B
% \]
% \[
%   \displaystyle A\mint{-}_{123}^{456} B
%   \textstyle A\mint{-}_{123}^{456} B
%   \scriptstyle A\mint{-}_{123}^{456} B
%   \scriptscriptstyle A\mint{-}_{123}^{456} B
% \]
% \[
%   \displaystyle A\mint{-}\limits_{12345}^{6} B
%   \textstyle A\mint{-}\limits_{12345}^{6} B
%   \scriptstyle A\mint{-}\limits_{12345}^{6} B
%   \scriptscriptstyle A\mint{-}\limits_{12345}^{6} B
% \]
% \[
%   \displaystyle A\mint{-}\limits_{1}^{23456} B
%   \textstyle A\mint{-}\limits_{1}^{23456} B
%   \scriptstyle A\mint{-}\limits_{1}^{23456} B
%   \scriptscriptstyle A\mint{-}\limits_{1}^{23456} B
% \]
% \[
%   \displaystyle A\mint{-}\displaylimits_{0}^{\infty} B
%   \textstyle A\mint{-}\displaylimits_{0}^{\infty} B
%   \scriptstyle A\mint{-}\displaylimits_{0}^{\infty} B
%   \scriptscriptstyle A\mint{-}\displaylimits_{0}^{\infty} B
% \]
% \[
%   \displaystyle A\mint{=} B
%   \textstyle A\mint{=} B
%   \scriptstyle A\mint{=} B
%   \scriptscriptstyle A\mint{=} B
% \]
% \[
%   \displaystyle A\mint{\equiv} B
%   \textstyle A\mint{\equiv} B
%   \scriptstyle A\mint{\equiv} B
%   \scriptscriptstyle A\mint{\equiv} B
% \]
% \[
%   \displaystyle A\mint{\circ} B
%   \textstyle A\mint{\circ} B
%   \scriptstyle A\mint{\circ} B
%   \scriptscriptstyle A\mint{\circ} B
% \]
%\end{document}
 

==> Sections/LDD-TPR_alternative_coupling_conditions.tex <==
It has been recognised in the literature since a long time that the interface conditions (\ref{eqn:LDD-TPR:ContinuousCouplingConditions:strong}), albeit being classical for domain decomposition formulations, fail to capture phenomena inherent to 
heterogeneous media, such as capillary trapping and more generally the experimentally observed  
discontinuity of pressures that possibly occur along soil layer boundaries of vastly different soil layers. 
For the full two phase flow model, aspects of this have been investigated 
more recently in \cite{Enchery2006,Brenner2011,Cances2012} 
building upon the earlier work in 
\cite{VanDuijn1995,Bertsch2003,Ersland1998}.
Cancès et al. formulate in \cite{Cances2012} coupling conditions admitting discontinuous pressures (moving phase conditions) along interfaces and prove the existence of a solution for this formulation.
    
The purpose of this section is twofold. 
First, we compare two different possibilities of enforcing moving phase conditions for a \TPR coupling and obtain a result on the jumping pressure regimes these two formulations encode. 
As a consequence of this considerations, one formulation clearly comes out as more capable of capturing the jumping pressure regimes. 
Notably, one version encodes moving phase conditions for both phases, whereas the other is a mixture of moving phase conditions for the wetting phase and pressure continuity for the nonwetting phase. 
Secondly, we envisage to develop an \LDD solver applicable to this situation. While an \LDD solver is formulated, no convergence analysis is provided, as our analytical tools employed so far, are inapt to handle the resulting formulation. 
Convergence of the proposed \LDDTPR solver with moving phase conditions remains an open question.

\subsection{Model considerations}

In order to formulate coupling conditions that capture pressure jumps possibly occurring at interfaces between soil layers 
with varying permeabilities and porosities, the relative permeabilities 
$\kaln{}$ must be allowed to become zero at their respective residual saturations $ \SalnNP{r} $.
In more detail, $\kaln{}\bigl( \SalnNP{r} \bigr) = 0$ for $\alpha = \nw,w$, where  $S_{\nw,l}^r = 1 - S_{w,l}^{\mbox{\scriptsize max}}$ 
and both $l\in \{1,2\}$. 
Here, $S_{w,l}^{\mbox{\scriptsize max}}$ is the maximal wetting saturation that can occur due to the residual saturation of the nonwetting phase.
Without 
loss of generality $S_{w,l}^r=S_{l}^r=0$ can be assumed%
\footnote{Since any compact interval $[a,b] \subset \RR$ can be diffeomorphically mapped to $[0,1]$, 
the relative permeabilities can be rescaled such that e.g. $\kwln{}(0) = 0$ translates to 
$\kwlnTilde{}(S_{l}^r) = 0$ and analogously for $\knwln{}$.}. 
Therefore , in what follows, we assume that $\kwln{}(0) = 0$ and $\knwln{}(1) = 0$. 
\begin{figure}[t]
  \centering
  \ifdevelopmentVersion
    \input{\LDDTPRfigSource/LDD-TPR-discontinuousPcAltConditions.tikz}
  \else
    \includegraphics[width=\textwidth]{Graphics/LDD-TwoPhaseRichards:LDD-TPR-discontinuousPcAltConditions}
  \fi
  \caption[\LDDTPRcaptionPrefix discontinuous $p_c$-curves, moving phase conditions]{ Illustration of discontinuous capillary pressure curves similar to the ones discussed in \cite{Enchery2006}, showing the uniquely defined saturations $S_l^*$, defining intervals in which phases can be trapped.  \label{fig:LDD-TPR:discontinuousPcAltCond} }
\end{figure}

The capillary pressure curves are assumed to behave as depicted in \autoref{fig:LDD-TPR:discontinuousPcAltCond}. 
In more detail, they are to be monotonically decreasing and as in \cite{Enchery2006}%
\footnote{Note, that as Enchery et al. use the nonwetting (oil) saturation for their formulation and analysis, by virtue of which monotonicities of relative permeabilities, $p_c$-curves and values for the saturations are reversed. We have adapted the presentation of the material to our notation.}, %
we assume that
\begin{align}
    p_{c,1}(1) \leq p_{c,2}(1) \leq p_{c,1}(0) \leq p_{c,2}(0).
    \label{eqn:LDD-TPR:altCond:Assumptions:pc1BelowPc2}
\end{align}
By $S_1^*$ and $S_2^*$, we denote the uniquely defined saturations in $[0,1]$, for which 
\begin{align}
    p_{c,1}(S_1^*) = p_{c,2}(1) \quad \mbox{and} \quad
    p_{c,2}(S_2^*) = p_{c,1}(0).
    \label{eqn:LDD-TPR:altCond:Assumptions:DefinitionOfTrappingSaturations}
\end{align}
As a consequence, for $s_1, s_2\in [0,S_2^*)$ and $\tilde{s}_1, \tilde{s}_2\in (S_1^*,1]$ we have the inequalities
\begin{align}
    p_{c,1}(s_1) < p_{c,2}(s_2) \quad \mbox{and} \quad
    p_{c,1}(\tilde{s}_1) < p_{c,2}(\tilde{s}_2).
    \label{eqn:LDD-TPR:altCond:Assumptions:pcInequelity}
\end{align}
In addition to the continuity of the normal component of  fluxes in (\ref{eqn:LDD-TPR:ContinuousCouplingConditions:strong}), 
the so-called \emph{moving phase} conditions 
\begin{align}
    \kaln[1]{}(S_{1})\pospartb{ \paln[1]{} - \paln[2]{} } &= \kaln[2]{}(S_{2})\pospartb{ \paln[2]{} - \paln[1]{}}, 
    \qquad \alpha \in\{w, \nw\}
    \label{eqn:LDD-TPR:ContinuousMovingPhaseConditions.strong}
\end{align}
are imposed on the interface instead of the continuity of the pressures, see \cite{Cances2012,Enchery2006}. 
$\pospart{f} = \max{ (f,0) }$ denotes the positive part of a function $f$. 
Equation (\ref{eqn:LDD-TPR:ContinuousMovingPhaseConditions.strong}) together with discontinuous capillary pressure curves encode regimes of saturations on each side of the interface in which either the pressures are continuous or a phase is missing (residual) on the side of the interface with higher pressure. 
For the \TPTP case, this is detailed in \cite{Enchery2006}. 

In case of a \TPR coupling, we have two possibilities of translating equation (\ref{eqn:LDD-TPR:ContinuousMovingPhaseConditions.strong}) to this setting. 
Assuming again the \Richards model on $\dom{1}$ and the full two-phase model on $\dom{2}$, equation
(\ref{eqn:LDD-TPR:ContinuousMovingPhaseConditions.strong}) remains meaningful for $\alpha = w$. However, for the nonwetting phase, we have two options. 
One standpoint would be that, since there is no equation for the 
nonwetting phase on $\dom{1}$, there should not be any relative permeability, replacing the relations in (\ref{eqn:LDD-TPR:ContinuousMovingPhaseConditions.strong}). 
Thus, one would have 
\begin{subequations}
\begin{align}
    \kwln[1]{}(S_{1})\pospartb{ \pwln[1]{} - \pwln[2]{} } &= \kwln[2]{}(S_{2})\pospartb{ \pwln[2]{} - \pwln[1]{}} 
    \label{eqn:LDD-TPR:MovingPhase.TPR.strong-wetting1} \\
    0 &= \knwln[2]{}(S_{2})\pospartb{ \pnwln[2]{} - \underbrace{p_a}_{=\pnwln[1]{}} }.
    \label{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting1} 
\end{align}
\end{subequations}
Recall, that $p_a$ denoted the atmospheric pressure.
Another possibility is to assume a relative permeability 
for the nonwetting phase, even though we do not model the phase with a full equation.  
Consequently, we prescribe the relations in (\ref{eqn:LDD-TPR:ContinuousMovingPhaseConditions.strong}) with the sole change of constant nonwetting pressure $\pnwln[1]{}=p_a$ on $\dom{1}$:
\begin{subequations}
\begin{align}
    \kwln[1]{}(S_{1})\pospartb{ \pwln[1]{} - \pwln[2]{} } &= \kwln[2]{}(S_{2})\pospartb{ \pwln[2]{} - \pwln[1]{}},
    \label{eqn:LDD-TPR:MovingPhase.TPR.strong-wetting2} \\
    \knwln[1]{}(S_{1})\pospartb{ p_a - \pnwln[2]{} } &= \knwln[2]{}(S_{2})\pospartb{ \pnwln[2]{} - p_a}.
    \label{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}
\end{align}
\end{subequations}
This is the approach corresponding to equation (\ref{eqn:LDD-TPR:ContinuousCouplingConditions:strong:alternative}) on page \pageref{eqn:LDD-TPR:ContinuousCouplingConditions:strong:alternative}.

In order to understand how both alternatives encode jumping pressures, and in what regard the conditions (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-wetting2}), (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}) and (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-wetting1}), (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting1}) differ from one another,   we follow the arguments presented in \cite{Enchery2006} and
obtain the following result.

\begin{proposition}[Pressure jump regimes of moving phase conditions for \TPR coupling]
    Assume that the monotonically decreasing capillary pressure curves $p_{c,1}$ and $p_{c,2}$ adhere to (\ref{eqn:LDD-TPR:altCond:Assumptions:pc1BelowPc2}), (\ref{eqn:LDD-TPR:altCond:Assumptions:DefinitionOfTrappingSaturations}) and (\ref{eqn:LDD-TPR:altCond:Assumptions:pcInequelity}). Then,
    \begin{enumerate}[label=\alph*)]
     \item the conditions 
        (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-wetting2}),  
        (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}) encode pressure jump regimes corresponding to \cite{Enchery2006} in the \TPTP case.
        In detail, we have:
        \begin{enumerate}[label=\roman*)]
            \item {\scshape Trapping of wetting phase in $\dom{2}$, mobile nonwetting phase, $p_a=p_{\nw,2}$.} \quad In case on $\dom{2}$ the wetting saturation fulfils $0\leq S_2 < S_2^*$, no wetting phase can occur on the $\dom{1}$-side of the interface $\interface$, i.e. $S_1=0$, and in addition the  entry pressure barrier
            \begin{align} 
                \pwln[2]{} <  \pwln[1]{},
            \end{align}
            occurs. 
            The pressure of the nonwetting phase is continuous, $p_a=p_{\nw,2}$, and the nonwetting phase is mobile.
            \item {\scshape Trapping of nonwetting phase in $\dom{1}$, mobile wetting phase $p_{w,1}=p_{w,2}$.} \quad In case on $\dom{1}$ the wetting saturation fulfils $S_1^*\leq S_1 < 1$, full saturation of the wetting phase must occur on the $\dom{2}$-side of $\interface$, i.e. $S_2=1$. 
            Consequently the nonwetting phase is absent on the $\dom{2}$-side of $\interface$, trapped on the $\dom{1}$-side and 
            an entry pressure barrier
            \begin{align} 
                p_a <  \pnwln[2]{},
            \end{align}
            occurs for the nonwetting phase. 
            The pressure of the wetting phase is continuous over the interface, $p_{w,1}=p_{w,2}$, and the phase is mobile.
            \item {\scshape No trapping, $p_{w,1}=p_{w,2}$ and $p_a=p_{\nw,2}$.} 
            In all other cases, $ S_2^*\leq S_2$ and $S_1 \leq S_1^*$, both phases are mobile over the interface and all pressures are continuous, i.e. 
            $p_{w,1}=p_{w,2}$, $p_a=p_{\nw,2}$ and a fortiori
            $p_{c,1}(S_1)=p_{c,2}(S_2)$. No trapping occurs and both phases are mobile over the interface.
        \end{enumerate}
        Notably, the continuity of the nonwetting pressure in the regimes where the nonwetting phase is mobile, is implicitly encoded in the conditions. 
    \item the conditions 
        (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-wetting1}),  
        (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting1})
        are in parts indecisive and encode the following
        \begin{enumerate}[label=\roman*)]
            \item {\scshape Trapping of wetting phase in $\dom{2}$, possible pressure jump $\pnwln[2]{}\leq p_a$.} \quad In case on $\dom{2}$ the wetting saturation fulfils $0\leq S_2 < S_2^*$, no wetting phase can occur on the $\dom{1}$-side of $\interface$, i.e. $S_1=0$, and in addition the entry pressure barrier
            \begin{align} 
                \pwln[2]{} <  \pwln[1]{},
            \end{align}
            occurs. For the nonwetting phase, we merely have $\pnwln[2]{}\leq p_a$ and the conditions in themselves do not contain enough information on the continuity of the nonwetting phase. A pressure jump might occur, or not. 
            \item {\scshape Trapping of nonwetting phase in $\dom{1}$, mobile wetting phase, $p_{w,1}=p_{w,2}$.} \quad In case on $\dom{1}$ the wetting saturation fulfils $S_1^*\leq S_1 < 1$, full saturation of the wetting phase must occur on the $\dom{2}$-side of $\interface$, i.e. $S_2=1$. 
            Consequently the nonwetting phase is absent on the $\dom{2}$-side of $\interface$, trapped on the $\dom{1}$-side and
            In addition, an entry pressure barrier
            \begin{align} 
                p_a <  \pnwln[2]{},
            \end{align}
            occurs. 
            The pressure of the wetting phase is continuous over the interface, $p_{w,1}=p_{w,2}$, and the phase is mobile.
            \item {\scshape Inconclusive for both phases.} 
            In all other cases, $ S_2^*\leq S_2$ and $S_1 \leq S_1^*$, the equations do not contain sufficient information to be conclusive. We have 
            $\pwln[2]{}\leq \pwln[1]{}$ and either 
            $k_{\nw,2}(S_2) = 0$ or $\pnwln[2]{}\leq p_a$.
            Only when $p_a=\pnwln[2]{}$ is assumed, e.g. as part of the notion of solution to the \TPR coupling, can we deduce $\pwln[1]{}=\pwln[2]{}$.
            In particular, the conditions do not infer the continuity of the capillary pressures 
            $p_{c,1}(S_1)=p_{c,2}(S_2)$ without assuming $p_a=\pnwln[2]{}$.
        \end{enumerate}
    \end{enumerate}
\end{proposition}

\begin{Proof}
\begin{enumerate}[label=\roman*)]
 \item Assume $0\leq S_2 < S_2^*$. %
    \label{enumerate:LDD-TPR:altCond:case:i}
    \begin{enumerate} 
        \item {\scshape Case (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-wetting2}),  
            (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}).} \quad
            Since $\knwln[2]{}(S_2) > 0$, by (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}) we must have 
            \begin{align} 
                \pnwln[2]{} \leq p_a.
                \label{eqn:LDD-TPR:altCond:pressureJump:case:i:pnw2Greaterpnw1}
            \end{align}
            Otherwise the left hand side of (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}) would be zero while the right hand side would not, yielding a contradiction. 
            Recall, that by (\ref{eqn:LDD-TPR:altCond:Assumptions:pcInequelity}), we know that 
            \begin{align*}
                p_a - \pwln[1]{} = p_{c,1}(S_1) \leq p_{c,1}(0) = p_{c,2}(S_2^*) < p_{c,2}(S_2) 
                    = \pnwln[2]{} - \pwln[2]{},
            \end{align*}
            which is the same as
                $p_a - \pnwln[2]{} - \pwln[1]{}  <  - \pwln[2]{}$,
            and thus 
            \begin{align} 
                \pwln[2]{} <  \pwln[1]{},
                \label{eqn:LDD-TPR:altCond:case:i:pressureJump:pw2Greaterpw1}
            \end{align} by virtue of $0 \leq p_a - \pnwln[2]{}$, (\ref{eqn:LDD-TPR:altCond:pressureJump:case:i:pnw2Greaterpnw1}).
            Taking (\ref{eqn:LDD-TPR:altCond:case:i:pressureJump:pw2Greaterpw1}) into account in (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-wetting2}), the right hand side of the latter vanishes. 
            Therefore $\kwln[1]{}(S_1)$ has to be zero as well, which is the case if $S_1 = 0$. This in turn means $\knwln[1]{}(S_1) > 0$ and therefore (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}) enforces 
            \begin{align}
                \pnwln[2]{} = p_a.
                \label{eqn:LDD-TPR:altCond:case:i:pressureEquality:nonwetting}
            \end{align}
            In this situation, the wetting phase is trapped in $\dom{2}$ and due to (\ref{eqn:LDD-TPR:altCond:case:i:pressureJump:pw2Greaterpw1}) there is a pressure barrier.  The nonwetting phase can flow across the interface and has continuous pressures. 
        \item {\scshape Case (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-wetting1}),
            (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting1}).} \quad
            All arguments presented in the above case remain valid except the last one using $\knwln[1]{}(S_1) > 0$, which yielded the pressure continuity of the nonwetting pressure (\ref{eqn:LDD-TPR:altCond:case:i:pressureEquality:nonwetting}). 
            Since we do not assume a nonwetting relative permeability $\knwln[1]{}$, in case we use (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting1}) instead of (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}), the coupling conditions contain no further information about the nonwetting pressure on $\dom{2}$. Thus, the possible inequality of the nonwetting pressures (\ref{eqn:LDD-TPR:altCond:pressureJump:case:i:pnw2Greaterpnw1}) remains, i.e. a pressure jump might also occur in the nonwetting phase.
            Note, however, that in the semi-discrete formulation of \autoref{env:LDD-TPR:problemFormulation:semiDiscrete:weak}, the pressure continuity of the nonwetting phase 
            (\ref{eqn:LDD-TPR:altCond:case:i:pressureEquality:nonwetting}) is enforced by requiring that $\pnwln[2]{n} \in H^1_0(\dom{2})$, so the coupling conditions do not need to reflect this. 
    \end{enumerate}
    Interestingly, using conditions
    (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-wetting2}),  
    (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}) instead enforces the continuity of the nonwetting pressures implicitly. 
\item Assume $ S_2^*\leq S_2$ and $S_1 \leq S_1^*$.
    \begin{enumerate} 
        \item {\scshape Case (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-wetting2}),  
            (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}).} \quad
            In this case we have 
            \begin{align}
                p_{c,2}(S_2) &\leq p_{c,2}(S_2^*) = p_{c,1}(0), 
                \label{eqn:LDD-TPR:altCond:case:ii:pc2lowerEqualPc1Zero}
                \\
                p_{c,2}(1)   &=    p_{c,1}(S_1^*) \leq p_{c,1}(S_1),
                \label{eqn:LDD-TPR:altCond:case:ii:pc2OnelowerEqualPc1}
            \end{align}
            as can be seen from Fig \ref{fig:LDD-TPR:discontinuousPcAltCond}.
            Because $\kwln[2]{}(S_2) > 0$, we know by (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-wetting2}) that 
            \begin{align} 
                \pwln[2]{} \leq \pwln[1]{} \quad &\mbox{and} \quad 
                \label{eqn:LDD-TPR:altCond:case:ii:pw2greaterEqualpw1}\\ 
                \kwln[1]{}(S_1) = 0 \quad &\mbox{or} \quad \pwln[2]{} = \pwln[1]{}.
                \label{eqn:LDD-TPR:altCond:case:ii:pressureEqualityOrS1zero}
            \end{align}
            Similarly, $\knwln[1]{}(S_1) > 0$, so that by (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}) we must have
            \begin{align} 
                p_a \leq \pnwln[2]{} \quad &\mbox{and} \quad 
                \label{eqn:LDD-TPR:altCond:case:ii:pagreaterEqualpnw2} \\ 
                \knwln[2]{}(S_2) = 0 \quad &\mbox{or} \quad \pnwln[2]{} = p_a.
                \label{eqn:LDD-TPR:altCond:case:ii:pressureEqualityOrS2zero}
            \end{align}
            Thereby, it must hold independently of (\ref{eqn:LDD-TPR:altCond:case:ii:pressureEqualityOrS1zero}) and
            (\ref{eqn:LDD-TPR:altCond:case:ii:pressureEqualityOrS2zero}) that
            $p_a - \pwln[1]{} \leq \pnwln[2]{} - \pwln[2]{}$, which is the same as
            \begin{align}
                p_{c,1}(S_1) \leq p_{c,2}(S_2).
                \label{eqn:LDD-TPR:altCond:case:ii:pc1lowerEqualPc2}
            \end{align}
            If we have $\kwln[1]{}(S_1) = 0$ in (\ref{eqn:LDD-TPR:altCond:case:ii:pressureEqualityOrS1zero}), i.e. $S_1=0$,
            equation (\ref{eqn:LDD-TPR:altCond:case:ii:pc1lowerEqualPc2}) together with (\ref{eqn:LDD-TPR:altCond:case:ii:pc2lowerEqualPc1Zero}) yields 
            \begin{align} 
                p_{c,1}(0) = p_{c,2}(S_2).
                \label{eqn:LDD-TPR:altCond:case:ii:pc1ZeroEqualPc2}
            \end{align}
            This together with the inequalities (\ref{eqn:LDD-TPR:altCond:case:ii:pw2greaterEqualpw1}) and (\ref{eqn:LDD-TPR:altCond:case:ii:pagreaterEqualpnw2}) (and independently of (\ref{eqn:LDD-TPR:altCond:case:ii:pressureEqualityOrS2zero})!) yields the continuity of all appearing pressures, for if, say (\ref{eqn:LDD-TPR:altCond:case:ii:pw2greaterEqualpw1}) was a strict inequality, we could deduce $p_a > \pnwln[2]{}$ from (\ref{eqn:LDD-TPR:altCond:case:ii:pc1ZeroEqualPc2}) in contradiction to (\ref{eqn:LDD-TPR:altCond:case:ii:pagreaterEqualpnw2}) and vice versa if (\ref{eqn:LDD-TPR:altCond:case:ii:pagreaterEqualpnw2}) is assumed to be strict. 
            
            Assume on the other hand we have $\pwln[1]{} = \pwln[2]{}$ in (\ref{eqn:LDD-TPR:altCond:case:ii:pressureEqualityOrS1zero}). Then either $p_a = \pnwln[2]{}$ by (\ref{eqn:LDD-TPR:altCond:case:ii:pressureEqualityOrS2zero}), i.e. all appearing pressures are continuous and thereby
            \begin{align} 
                p_{c,1}(S_1) = p_{c,2}(S_2),
                \label{eqn:LDD-TPR:altCond:case:ii:pc1EqualPc2}
            \end{align}
            or we have $\knwln[2]{}(S_2) = 0$, which means $S_2=1$. 
            Thus, 
            inequality (\ref{eqn:LDD-TPR:altCond:case:ii:pc1lowerEqualPc2}) together with (\ref{eqn:LDD-TPR:altCond:case:ii:pc2OnelowerEqualPc1}) yields 
            \begin{align}
                p_{c,1}(S_1) = p_{c,2}(1)
            \end{align} 
            and thereby we have 
            $p_a = \pnwln[2]{}$ as well.
            
            In summary, we have $p_{c,1}(S_1) = p_{c,2}(S_2)$ as well as $\pwln[1]{} = \pwln[2]{}$ and $p_a = \pnwln[2]{}$ under the assumption $ S_2^*\leq S_2$ and $S_1 \leq S_1^*$. This means that both phases flow across the interface and no trapping occurs.
            
            

        \item {\scshape Case (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-wetting1}),
            (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting1}).} \quad
            Equations (\ref{eqn:LDD-TPR:altCond:case:ii:pc2lowerEqualPc1Zero})–(\ref{eqn:LDD-TPR:altCond:case:ii:pressureEqualityOrS1zero}) stay the same. However, replacing (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}) by (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting1}), we cannot deduce (\ref{eqn:LDD-TPR:altCond:case:ii:pagreaterEqualpnw2}) anymore and instead merely get
            \begin{align} 
                \knwln[2]{}(S_2) = 0 \quad &\mbox{or} \quad \pnwln[2]{} \leq p_a
                \tag{\ref{eqn:LDD-TPR:altCond:case:ii:pressureEqualityOrS2zero}'}
                \label{eqn:LDD-TPR:altCond:case:ii:pressureEqualityOrS2zero2}
            \end{align}
            from (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting1}). 
            As a consequence, we can deduce (\ref{eqn:LDD-TPR:altCond:case:ii:pc1lowerEqualPc2}) only in case $\pnwln[2]{} = p_a$ in (\ref{eqn:LDD-TPR:altCond:case:ii:pressureEqualityOrS2zero2}). 
            In that particular instance, the capillary pressures and the phase pressures are again continuous for both cases of (\ref{eqn:LDD-TPR:altCond:case:ii:pressureEqualityOrS1zero}). 
            If $\knwln[2]{}(S_2) = 0$ in (\ref{eqn:LDD-TPR:altCond:case:ii:pressureEqualityOrS2zero2}), we have neither information on 
            the behaviour of the $p_c$ curves nor on the behaviour of the nonwetting pressure $\pnwln[2]{}$. 
            A jump might occur, or not. 
            In case the inequality in (\ref{eqn:LDD-TPR:altCond:case:ii:pressureEqualityOrS2zero2}) is strict, we know that 
            the nonwetting pressures cannot be continuous, i.e. due to $\pnwln[2]{} < p_a$ a pressure jump occurs. However, the behaviour of the $p_c$ curves is inconclusive.
            
            Note that if we adhere again to the notion of solution in the semi-discrete formulation of \autoref{env:LDD-TPR:problemFormulation:semiDiscrete:weak}, the pressure continuity of the nonwetting phase $\pnwln[2]{} = p_a$ is enforced by requiring that $\pnwln[2]{n} \in H^1_0(\dom{2})$ (after normalising $p_a$ to zero).
            In this case we again have both the continuity of the capillary pressures and phase pressures in accordance with ii) a).
    \end{enumerate}
\item Assume $ S_1^* < S_1 \leq 1$.
    \begin{enumerate} 
        \item {\scshape Case (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-wetting2}),  
            (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}).} \quad
            This case is strongly analogous to \ref{enumerate:LDD-TPR:altCond:case:i}. 
            Since $\kwln[1]{}(S_1) > 0$, by (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-wetting2}) we must have 
            \begin{align} 
                \pwln[1]{} \leq \pwln[2]{}.
                \label{eqn:LDD-TPR:altCond:pressureJump:case:iii:pw1Greaterpw2}
            \end{align}
            By (\ref{eqn:LDD-TPR:altCond:Assumptions:pcInequelity}), we know that 
            \begin{align*}
                p_a - \pwln[1]{} = p_{c,1}(S_1) < p_{c,1}(S_1^*) = p_{c,2}(1) \leq p_{c,2}(S_2) 
                    = \pnwln[2]{} - \pwln[2]{},
            \end{align*}
            which is the same as
                $p_a  - (\pwln[1]{}- \pwln[2]{}) < \pnwln[2]{} $,
            and thus 
            \begin{align} 
                p_a <  \pnwln[2]{},
                \label{eqn:LDD-TPR:altCond:case:iii:pressureJump:pnw2Greaterpa}
            \end{align} by virtue of (\ref{eqn:LDD-TPR:altCond:pressureJump:case:iii:pw1Greaterpw2}).
            Taking (\ref{eqn:LDD-TPR:altCond:case:iii:pressureJump:pnw2Greaterpa}) into account in (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2})
            enforces $\knwln[2]{}(S_2)=0$, thusly $S_2 = 1$ due to the vanishing left hand side of (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}). This in turn means $\kwln[2]{}(S_2) > 0$ and therefore (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-wetting2}) enforces 
            \begin{align}
                \pwln[2]{} = \pwln[1]{}.
                \label{eqn:LDD-TPR:altCond:case:iii:pressureEquality:wetting}
            \end{align}
            In this situation, the nonwetting phase is trapped in $\dom{1}$ and due to (\ref{eqn:LDD-TPR:altCond:case:iii:pressureJump:pnw2Greaterpa}) there is an entry pressure barrier for this phase to enter $\dom{2}$.  The wetting phase can flow freely over the interface and has continuous pressures. 
        \item {\scshape Case (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-wetting1}),
            (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting1}).} \quad
            The arguments in a) go through in this case since the left hand side of (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}) vanishes due to  (\ref{eqn:LDD-TPR:altCond:case:iii:pressureJump:pnw2Greaterpa}).  Thus, the existence of $\knwln[1]{}$ in the arguments in a) is irrelevant and (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}) might very well be replaced by 
            (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting1}) without affecting the outcome.
    \end{enumerate}
\end{enumerate}
\end{Proof}
\begin{corollary}[Equivalence of moving phase conditions \TPR coupling]~
\label{corollary:LDD-TPR:equivalenceOfMovingPhase}
  \begin{enumerate}[label=\roman*)]
    \item For a tuple of functions $(\pwln[1]{n},\pwln[2]{n},\pnwln[2]{n}) \in \dFs\times H^1_0(\dom{2})$ 
    solving equations (\ref{LDD-TPR:limitsystemeRichards})–(\ref{LDD-TPR:limitsystemeqn1nw}) of \autoref{env:LDD-TPR:problemFormulation:semiDiscrete:weak}, using equations 
    (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-wetting1}) and (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting1})
    instead of
    (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-wetting2}) and (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}) 
    as moving phase conditions yields the same jumping pressure regimes. 
    Both formulations encode the same type of trapping behaviour as in the \TPTP case explained in \cite{Enchery2006}. 
    \item For a tuple of functions $(\pwln[1]{n},\pwln[2]{n},\pnwln[2]{n}) \in \dFs\times \Fs_2$ 
    solving (\ref{LDD-TPR:limitsystemeRichards})–(\ref{LDD-TPR:limitsystemeqn1nw}) of \autoref{env:LDD-TPR:problemFormulation:semiDiscrete:weak}, imposing  
    (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-wetting2}) and (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}) 
    as moving phase conditions encodes the pressure jump regimes as i). Notably, the coupling conditions implicitly enforce the continuity of the nonwetting pressures $p_a=\pnwln[2]{}$  for all cases in which the nonwetting phase is mobile over the interface.
    The conditions (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-wetting1}) and (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting1}) by contrast, are inconclusive in this situation.
  \end{enumerate}\vspace{-5ex}
\end{corollary}
\begin{remark}
    In view of the above discussion the conditions (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-wetting2}) and (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}) allow to weaken the requirements for the notion of solution of a \TPR coupling with moving phase boundary conditions. Namely, the hard-coded continuity of nonwetting pressures resulting from demanding $\pnwln[2]{n}$ to be in $\in H^1_0(\dom{2})$, can be relaxed. 
    In addition, requiring $\pnwln[2]{n} \in  H_0^1(\dom{1})$ corresponds to having a fixed continuity requirement for the nonwetting phase and a moving phase type condition for the wetting phase, which is a mixture of both.
\end{remark}



\subsection{\LDD considerations for moving phase conditions.}
We have already mentioned in \autoref{remark:LDD-TPR:discussionCouplingConditions} \ref{remark:LDD-TPR:discussionCouplingConditions:discontinuousPc}, p. \pageref{remark:LDD-TPR:discussionCouplingConditions}, that due to the work of \cite{Cances2012}, the situation described by the discontinuous pressure curves along with the moving phase conditions can be approximated by replacing the discontinuous capillary  pressure curves by a pair of matching ones and use the \LDDTPR scheme given by \autoref{definition:LDD-TPR:solverAndScheme} and \autoref{env:LDD-TPR:LDD-scheme:weak}.  In the limit of a regularisation parameter ($\tilde{n}$ in \autoref{remark:LDD-TPR:discussionCouplingConditions}), the matching curves tend to the actual curves, and thus the \LDDTPR scheme becomes a possible approximation. 

In order to reflect discontinuous pressures along with moving phase conditions in a possible \LDD scheme explicitly, we first need to reformulate the problem we are approximating in terms of slightly different 
spaces and a generalised coupling condition.  

For $l=1,2$, let  $G_l : \Ts[]{}  \times \Ts[]{} \longrightarrow \Tracespace' $ be 
arbitrary functions of the traces of the pressures on the interface taking values in
$\dualTs[00]{}$. We assume, that the coupling conditions of interest can be cast into the generic form
\begin{align}
    \Glwone{} &= \Glwtwo{} && \mbox{in } \Tracespace'.  \label{eqn:LDD-TPR:GenericCouplingConditions}
\end{align}
Both the pressure continuity assumption of \autoref{env:LDD-TPR:problemFormulation:semiDiscrete:weak} 
as well as the moving phase conditions (\ref{eqn:LDD-TPR:ContinuousMovingPhaseConditions.strong}) 
fall into this category: 
To prescribe \emph{pressure continuity}, choose 
\begin{align}
    \Gla{} = \onGamma{\paln[l]{}}
\end{align}
and for the \emph{moving phase conditions}, choose 
\begin{align}
    \Gla{} = \onGamma{\kaln{}(S_l)\pospartb{ \paln[l]{} - \paln[3-l]{} }}.
\end{align}
 In all these cases, we understand these traces as functionals in $\Tracespace'$ via the $\Tracespace$-scalar product in line with \autoref{note:LDD-TPR:pressureFunctionalsDefiniton}.
With this notation, the generalised semi-discrete problems read as follows. 

\begin{problem}[\TPTP with moving phase conditions]~
\label{env:LDD-TPR:DiscontiuousProblemFormulation:TPTP:semiDiscrete:weak} 
For $l\in \{1,2\}$ and $\alpha\in\{w, \nw\}$, let $(\paln[1]{n-1},\paln[2]{n-1})$ $\in$ $\dFs$ and
\begin{align} 
    \Gla{n} = \onGamma{\kaln{n}\pospartb{ \paln[l]{n} - \paln[3-l]{n} }}
\end{align}
be given.  

Find $(\paln[1]{n},\paln[2]{n})$ $\in$ $\dFs$, such that $\fluxn[l]{\alpha}\cdot \vt{n_l} \in \dualTs[00]{} $ 
and the equations
  \begin{align}
     (-1)^{\krond{\nw}}\spl S_1^{n} - S_1^{n-1},\testfunc[1]{\alpha}\spr  %
      &- \tau\spl \fluxn[1]{\alpha},\bm{\nabla}\testfunc[1]{\alpha} \spr \nonumber \\
      &+ \tau \spl \fluxn[2]{\alpha}\cdot \vt{n_1},\testfunc[1]{\alpha}\spr_\Gamma 
      =  \tau\spl  f_{\alpha,1}^n ,\testfunc[1]{\alpha} \spr, 
      \label{eqn:LDD-TPR:DiscontiuousLimitSystemeTwoPhase:Dom1} \\
     (-1)^{\krond{\nw}}\spl S_2^{n} - S_2^{n-1},\testfunc[2]{\alpha}\spr  %
      &- \tau\spl \fluxn[2]{\alpha},\bm{\nabla}\testfunc[2]{\alpha} \spr \nonumber \\
      &+ \tau \spl \fluxn[1]{\alpha}\cdot \vt{n_2},\testfunc[2]{\alpha}\spr_\Gamma 
      =  \tau\spl  f_{\alpha,2}^n ,\testfunc[2]{\alpha} \spr,
       \label{eqn:LDD-TPR:DiscontiuousLimitSysteme:TwoPhase:Dom2} \\ %
     \Glaone{n}  	&= 	\Glatwo{n}
     \qquad\qquad\qquad\mbox{in } \Tracespace' \label{eqn:LDD-TPR:DiscontiuousLimitSysteme:TPTP:GContinuity}
  \end{align}
  are satisfied for both phases $\alpha\in\{w,\nw\}$ and for all $(\testfunc[1]{\alpha},\testfunc[2]{\alpha}) \in \dFs$.
\end{problem}%

Similarly, taking Corollary \ref{corollary:LDD-TPR:equivalenceOfMovingPhase} into account, the \TPR coupling reads as follows. 
\begin{problem}[\TPR with moving phase conditions]~
\label{env:LDD-TPR:DiscontiuousProblemFormulation:TPR:semiDiscrete:weak} 
Given $(\pwln[1]{n-1},\pwln[2]{n-1})$ $\in$ $\dFs$ and $\pnwln[2]{n-1}$ $\in$ $H_0^1(\dom{2})$, 
let
\begin{align}
    \Gla{n} := \onGamma{\kaln{n}\pospartb{ \paln[l]{n} - \paln[3-l]{n} }}
\end{align}
be given for 
$(\alpha, l) \in \{(w,1), (w,2), (\nw,2)\}$ as well as either 
\begin{align} 
    \Glnwone{n} := \onGamma{\knwln[1]{n}\pospartb{- \pnwln[2]{n} }} \quad \mbox{ or } \quad
    \Glnwone{n} := 0
\end{align}
depending on wether (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}) or 
(\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting1}) is taken into account.

Find $(\pwln[1]{n},\pwln[2]{n},\pnwln[2]{n}) \in \dFs \times H_0^1(\dom{1})$ in case 
(\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting1}) is assumed and 
$(\pwln[1]{n},\pwln[2]{n}$, $\pnwln[2]{n}) \in \dFs \times \Fs_2$, if (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}) is used, all the while setting  $\pnwln[1]{n}:=0$, such that $\fluxn[l]{\alpha}\cdot \vt{n_l} \in \dualTs[00]{} $ for $l=1,2$ and $\alpha\in\{w, \nw\}$ %
and the equations 
  \begin{align}
     \spl S_1^{n} - S_1^{n-1},\testfunc[1]{w}\spr  %
      &- \tau\spl \fluxn[1]{w},\bm{\nabla}\testfunc[1]{w} \spr \nonumber \\
      &+ \tau \spl \fluxn[2]{w}\cdot \vt{n_1},\testfunc[1]{w}\spr_\Gamma 
      =  \tau\spl  f_{w,1}^n ,\testfunc[1]{w} \spr,
      &&  \label{eqn:LDD-TPR:DiscontiuousLimitSystemeRichards} \\
     \spl S_2^{n} - S_2^{n-1},\testfunc[2]{w}\spr  %
      &- \tau\spl \fluxn[2]{w},\bm{\nabla}\testfunc[2]{w} \spr \nonumber \\
      &+ \tau \spl \fluxn[1]{w}\cdot \vt{n_2},\testfunc[2]{w}\spr_\Gamma 
      =  \tau\spl  f_{w,2}^n ,\testfunc[2]{w} \spr,
      &&  \label{eqn:LDD-TPR:DiscontiuousLimitSysteme:TwoPhase:wetting} %
    \end{align}
    together with
    \begin{align}
     \Glwone{n}  	&= 	\Glwtwo{n}
     && \mbox{in } \Tracespace' \label{eqn:LDD-TPR:DiscontiuousLimitSysteme:TPR:GContinuity:wetting}
     \end{align}
     and 
     \begin{align}
    -\spl S_2^{n} - S_2^{n-1},\testfunc[2]{\nw}\spr  %
      &- \tau\spl \fluxn[2]{\nw},\bm{\nabla}\testfunc{\nw} \spr \nonumber \\
      &+ \tau \spl \fluxn[1]{\nw}\cdot \vt{n_2},\testfunc[2]{\nw}\spr_{\Gamma}
      =  \tau\spl  f_{\nw,2}^n ,\testfunc[2]{\nw} \spr \label{eqn:LDD-TPR:DiscontiuousLimitSysteme:TwoPhase:nonwetting}
      \end{align}
      together with 
      \begin{align}
        \Glnwone{n}  	&= 	\Glnwtwo{n}
     && \mbox{in } \Tracespace' \label{eqn:LDD-TPR:DiscontiuousLimitSysteme:TPR:GContinuity:nonwetting}
  \end{align}
  are satisfied for all $(\testfunc[1]{w},\testfunc[2]{w}) \in \dFs$ and $\testfunc[2]{\nw} \in \Fs_2$.
\end{problem}%

\subsubsection{Limit systems for \TPTP and \TPR with moving phase conditions}
Following the discussion that lead to the reformulation 
(\ref{eqn:LDD-TPR:limitSystem:wetting})–(\ref{eqn:LDD-TPR:limitSystem:gli:nonwetting:2}) of 
\autoref{env:LDD-TPR:problemFormulation:semiDiscrete:weak}, we rewrite Problems \ref{env:LDD-TPR:DiscontiuousProblemFormulation:TPTP:semiDiscrete:weak} and 
\ref{env:LDD-TPR:DiscontiuousProblemFormulation:TPR:semiDiscrete:weak} accordingly into possible limit systems.

For a solution $\bigl( (\pwln[1]{n}, \pwln[2]{n}), \pnwln[2]{n} \bigr)$ of 
\autoref{env:LDD-TPR:DiscontiuousProblemFormulation:TPR:semiDiscrete:weak} or a solution 
$(\paln[1]{n}, \paln[2]{n})$, $\alpha \in \{n, \nw\}$ of 
\autoref{env:LDD-TPR:DiscontiuousProblemFormulation:TPTP:semiDiscrete:weak}, the functionals 
\begin{align}
  \gali{} &:= -\Gla{n} + \fluxn{\alpha}\cdot \vt{n_l}, && l\in \{1,2\},\,\, \alpha \in \{n, \nw\} \label{LDD-TPR:eqn:galn:discontiuous:alpha} %
\end{align}
in $\Tracespace'$ fulfil the relations
\begin{align}
  \gali{} %
      &= -2\Gtmla{n} + \Gtmla{n} - \fluxn[3-l]{\alpha}\cdot \vt{n_{3-l}} \nonumber \\
      &= -2\Gtmla{n} - \gali[3-l]{}&& 
\end{align}
for $l=1,2$ and $\alpha \in \{n, \nw\}$, by virtue of the continuity of fluxes implicit to both formulations.
Using these relations, Problems \ref{env:LDD-TPR:DiscontiuousProblemFormulation:TPTP:semiDiscrete:weak} and \ref{env:LDD-TPR:DiscontiuousProblemFormulation:TPR:semiDiscrete:weak} can therefore  be rewritten into the following two formulations.
\begin{problem}[Formal limit system \TPR with generalised coupling conditions]
\label{problem:LDD-TPR:limitsystem:TPR:movingPhase}
Find $(\pwln[1]{n},\pwln[2]{n},\pnwln[2]{n}) \in \dFs \times H_0^1(\dom{1})$ in case 
(\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting1}) is assumed or 
$(\pwln[1]{n},\pwln[2]{n}$, $\pnwln[2]{n}) \in \dFs \times \Fs_2$ if (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}) is used, and $\gal{}\in \Tracespace'$ for all $l\in\{1,2\}$ and $\alpha\in\{w, \nw\}$, with $\gnwl[1]{}$ correspondingly given by either 
(\ref{eqn:LDD-TPR:gl0withoutGravity}) or (\ref{eqn:LDD-TPR:gl0withGravity}),
such that the equations
\begin{align}
   \spl S_l^{n} - S_l^{n-1},\testfunc{w}\spr  %
    &- \tau\spl \fluxb[n]{w},\bm{\nabla}\testfunc{w} \spr \nonumber \\
    &+ \tau \spl \Glw{n}
    + \gwl,\testfunc{w}\spr_\interface
    =  \tau\spl  f_{w,l}^n ,\testfunc{w} \spr \tag{\ref{eqn:LDD-TPR:DiscontiuousLimitSystemeRichards}'} 
    \label{eqn:LDD-TPR:limitSystem:TPR:discontinuous:wetting}
\end{align}
and 
\begin{align}
  \spl \gwl,\testfunc{w}\spr_{\interface}  
  =\spl -2\Gtmlw{n} -   \gwl[3-l]{},\testfunc{w}\spr_{\interface}
  \label{eqn:LDD-TPR:limitSystem:TPR:discontinuous:gliupdate:wetting}
\end{align}
hold for the wetting phase and both subdomains $\dom{l}$, $l\in\{1,2\}$, as well as 
\begin{align}
  -\spl S_2^{n} - S_2^{n-1},&\testfunc[2]{\nw}\spr  %
    - \tau\spl \fluxn[2]{\nw},\bm{\nabla}\testfunc[2]{\nw} \spr \nonumber \\
    &+ \tau \spl \Glnwtwo{n}
    + \gnwl[2]{} ,\testfunc[2]{\nw}\spr_\interface
    =  \tau\spl  f_{\nw,2}^n ,\testfunc[2]{\nw} \spr \tag{\ref{eqn:LDD-TPR:DiscontiuousLimitSysteme:TwoPhase:nonwetting}'}\label{eqn:LDD-TPR:limitSystem:TPR:discontinuous:nonwetting} 
\end{align}
together with
\begin{align}
    \spl \gnwl[1]{},\testfunc[2]{\nw}\spr_{\interface} 
      &=\spl -2\Glnwtwo{n}-\gnwl[2]{},\testfunc[2]{\nw}\spr_{\interface}, 
        \label{eqn:LDD-TPR:limitSystem:TPR:discontinuous:gli:nonwetting:1}\\
      \spl \gnwl[2]{},\testfunc[2]{\nw}\spr_{\interface} 
       &=\spl -2\Glnwone{n} -\gnwli[1]{},\testfunc[2]{\nw}\spr_{\interface} 
    \label{eqn:LDD-TPR:limitSystem:gli:TPR:discontinuous:nonwetting:2}
\end{align}
are fulfilled for the nonwetting phase for all $(\testfunc[1]{w}, \testfunc[2]{w}) \in \dFs$ and 
$\testfunc[1]{\nw} \in \Fs_2$.
\end{problem}
\begin{problem}[Limit system for \TPTP with generalised coupling conditions]
\label{problem:LDD-TPR:limitsystem:TPTP:movingPhase}
Find $\bigl( \paln[1]{n}, \paln[2]{n}\bigr)\in \dFs$ and $\gal{}\in \Tracespace'$ for $l\in\{1,2\}$ and $\alpha\in\{w, \nw\}$, 
such that the equations
\begin{align}
   \spl S_l^{n} - S_l^{n-1},&\testfunc{w}\spr  %
    - \tau\spl \fluxb[n]{w},\bm{\nabla}\testfunc{w} \spr \nonumber \\
    &+ \tau \spl \Glw{n}
    + \gwl,\testfunc{w}\spr_\interface
    =  \tau\spl  f_{w,l}^n ,\testfunc{w} \spr
    \label{eqn:LDD-TPR:limitSystem:TPTP:discontinuous:wetting} 
\end{align}
and
\begin{align}
  \spl \gwl,\testfunc{w}\spr_{\interface}  
  =\spl -2\Gtmlw{n} -   \gwl[3-l]{},\testfunc{w}\spr_{\interface}, 
  \label{eqn:LDD-TPR:limitSystem:TPTP:discontinuous:gliupdate:wetting}
\end{align}
as well as 
\begin{align}
  -\spl S_l^{n} - S_l^{n-1},&\testfunc[l]{\nw}\spr  %
    - \tau\spl \fluxn[l]{\nw},\bm{\nabla}\testfunc[l]{\nw} \spr \nonumber \\
    &+ \tau \spl G_l(\pnwln[1]{n}, \pnwln[2]{n})
    + \gnwl[l]{} ,\testfunc[l]{\nw}\spr_\interface
    =  \tau\spl  f_{\nw,l}^n ,\testfunc[l]{\nw} \spr 
    \label{eqn:LDD-TPR:limitSystem:TPTP:discontinuous:nonwetting} 
\end{align}
together with
\begin{align}
      \spl \gnwl[l]{},&\testfunc[l]{\nw}\spr_{\interface} 
      =\spl -2\Gtmlnw{n}-\gnwl[3-l]{},\testfunc[l]{\nw}\spr_{\interface}, 
      \label{eqn:LDD-TPR:limitSystem:TPTP:discontinuous:gli:nonwetting}
\end{align}
are fulfilled for $l\in\{1, 2\}$ and all $\bigl(\testfunc[1]{\alpha}, \testfunc[2]{\alpha}\bigr) \in \dFs$.
\end{problem}

Repeating the exact same arguments 
in the proof of \autoref{lemma:LDD-TPR:iterationinterpretationlemma}, p. \pageref{lemma:LDD-TPR:iterationinterpretationlemma},
shows that conversely, any functions 
$\bigl((\pwln[1]{n}, \pwln[2]{n}), \pnwln[2]{n}\bigr) \in \dFs\times H^1_0(\dom{2})$ or  
$\bigl((\pwln[1]{n}, \pwln[2]{n}),$ $\pnwln[2]{n}\bigr) \in \dFs\times\Fs_2$ 
that fulfil 
\autoref{problem:LDD-TPR:limitsystem:TPR:movingPhase}
also solve Problem 
\ref{env:LDD-TPR:DiscontiuousProblemFormulation:TPR:semiDiscrete:weak}.
Analogously, a solution $(\paln[1]{n}, \paln[2]{n}) \in \Fs_1\times\Fs_2$ to 
\autoref{problem:LDD-TPR:limitsystem:TPTP:movingPhase}
solves Problem 
\ref{env:LDD-TPR:DiscontiuousProblemFormulation:TPTP:semiDiscrete:weak}.

\subsubsection{A possible \LDD solver for moving phase conditions} 
As in the case of continuous pressures, the reformulations of the Problems
\ref{env:LDD-TPR:DiscontiuousProblemFormulation:TPR:semiDiscrete:weak}
and 
\ref{env:LDD-TPR:DiscontiuousProblemFormulation:TPTP:semiDiscrete:weak}
into Problem
\ref{problem:LDD-TPR:limitsystem:TPR:movingPhase} and \ref{problem:LDD-TPR:limitsystem:TPTP:movingPhase}
suggest a formulation of an \LDD solver having these formulations as limit systems.
Again, the \LDD solver is introduced to linearise and decouple the problem in one step. However, the new conditions 
(\ref{eqn:LDD-TPR:DiscontiuousLimitSysteme:TPTP:GContinuity}) and
(\ref{eqn:LDD-TPR:DiscontiuousLimitSysteme:TPR:GContinuity:wetting}), (\ref{eqn:LDD-TPR:DiscontiuousLimitSysteme:TPR:GContinuity:nonwetting})
introduce a (nonlinear) coupling of their own, which needs to be addressed.

Accordingly, we propose:

\begin{problem}[\LDDTPR solver step for \TPR with moving phase conditions] \label{env:LDD-TPR:LDD-scheme:AltCond:weak}
For some $L_{\alpha,2},L_{w,1} > 0$, $\alpha\in\{w, \nw\}$ and $l\in\{1,2\}$, let the previous iterates
$\pwlni{i-1} \in \Fs_l$ and either $\pnwlni[2]{i-1} \in \Fs_2$ in case 
(\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}) is assumed or $\pnwlni[2]{i-1} \in H^1_0(\dom{2})$ in case 
(\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting1}) is used be known together with $\gali{i-1}\in \Tracespace'$,  $(\NN\in i \geq 1)$. 
Then, one step of the \LDD solver consists of 
finding 
$(\pwlni[1]{i},\pwlni[2]{i},\pnwlni[2]{i}) \in \dFs \times H_0^1(\dom{1})$ in case 
(\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting1}) is assumed and 
$(\pwlni[1]{i},\pwlni[2]{i},\pnwlni[2]{i}) \in \dFs \times \Fs_2$, if (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}) is used
such that the equations
\begin{align}
  L_{w,l}\spl &\pwlni{i},\testfunc{w} \spr
    - \tau\spl \fluxwi{i},\bm{\nabla}\testfunc{w} \spr \nonumber \\
    &+ \tau \spl \lambda_w \kwlni{i} \pospartb{ \onGamma{\pwlni{i}}  - \onGamma{\pwlni[3-l]{i-1}} }
    + \gwli{i} ,\testfunc{w}\spr_\interface  \nonumber \\
  &\qquad= L_{w,l}\spl \pwlni{i-1},\testfunc{w}\spr
      - \spl S_l^{n,i-1} - S_l^{n-1},\testfunc{w}\spr
    + \tau\spl  f_{w,l}^n ,\testfunc{w} \spr,
      \label{eqn:LDD-TPR:AltCond:TPR:wetting}	
\end{align}
with
\begin{align}
  \spl &\gwli{i},\testfunc{w}\spr_{\interface}  :=
  \spl -2\lambda_{w} \kwlni[3-l]{i-1}
  \pospartb{ \onGamma{\pwlni[3-l]{i-1}} - \onGamma{\pwlni[l]{i-2}} } -   \gwli[3-l]{i-1},\testfunc{w}\spr_{\Gamma}, 	 \label{eqn:LDD-TPR:AltCond:gliUpdate:wetting}
  \end{align}
hold for $l\in \{1,2\}$ and the equations
  \begin{align}
  L_{\nw,2}&\spl \pnwlni[2]{i},\testfunc[2]{\nw} \spr
    - \tau\spl \fluxgi[2]{i},\bm{\nabla}\testfunc[2]{\nw} \spr \nonumber \\
    &+ \tau \spl \lambda_{\nw} \knwlni[2]{i} \pospartb{ \onGamma{\pnwlni[2]{i}}}
    + \gnwli[2]{i} ,\testfunc[2]{\nw}\spr_\interface \nonumber \\
  &\quad= L_{\nw,2}\spl \pnwlni[2]{i-1},\testfunc[2]{\nw}\spr
      +  \spl S_2^{n,i-1} - S_2^{n-1},\testfunc[2]{\nw}\spr
    + \tau\spl  f_{\nw,2}^n ,\testfunc[2]{\nw} \spr \label{eqn:LDD-TPR:AltCond:TPR:nonwetting}
\end{align}
together with
\begin{align}
    \spl &\gnwli[1]{i},\testfunc[2]{\nw}\spr_{\interface} 
      :=\spl -2\lambda_{\nw} \knwlni[2]{i-1}
  \pospartb{ \onGamma{\pnwlni[2]{i-1}} }-\gnwli[2]{i-1},\testfunc[2]{\nw}\spr_{\interface}, \label{eqn:LDD-TPR:AltCond:gliUpdate:nonwetting:weak:1}
  \end{align}
  and either 
  \begin{align}
        \spl &\gnwli[2]{i},\testfunc[2]{\nw}\spr_{\interface} 
       :=\spl -\gnwli[1]{i-1},\testfunc[2]{\nw}\spr_{\interface}, \label{eqn:LDD-TPR:AltCond:gliUpdate:nonwetting:weak:2a}
\end{align}
or 
\begin{align}
       \spl &\gnwli[2]{i},\testfunc[2]{\nw}\spr_{\interface} 
       :=\spl -2\lambda_{\nw} \knwlni[1]{i-1}
  \pospartb{ -\onGamma{\pnwlni[2]{i-2}} } -\gnwli[1]{i-1},\testfunc[2]{\nw}\spr_{\interface}, 
  \tag{\ref{eqn:LDD-TPR:AltCond:gliUpdate:nonwetting:weak:2a}'}\label{eqn:LDD-TPR:AltCond:gliUpdate:nonwetting:weak:2b}
\end{align}
are fulfilled for all $(\testfunc[1]{w},\testfunc[2]{w})\in \dFs$ and $\testfunc[2]{\nw} \in \Fs_{2}$.
Here, imposing (\ref{eqn:LDD-TPR:AltCond:gliUpdate:nonwetting:weak:2a}) corresponds modelling according to 
(\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting1}), i.e. not assuming any relative permeability 
and (\ref{eqn:LDD-TPR:AltCond:gliUpdate:nonwetting:weak:2b}) corresponds 
(\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}), where a relative permeability is assumed for the nonwetting phase on $\dom{1}$.
\end{problem}
The solver can analogously be formulated for the \TPTP coupling.
\begin{remark}
    In case this proposed \LDD scheme converges to a solution of  (\ref{eqn:LDD-TPR:limitSystem:TPTP:discontinuous:wetting})–(\ref{eqn:LDD-TPR:limitSystem:TPTP:discontinuous:gli:nonwetting}) and the coupling conditions according to (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting1}) have been assumed, the limit fulfils (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-wetting1}) and (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting1}). In view of the discussion leading to Corollary \ref{corollary:LDD-TPR:equivalenceOfMovingPhase}, these conditions do not imply the continuity of the nonwetting pressure in case the nonwetting phase is mobile. As a consequence, it seems necessary, to impose the requirement
    $(\pwlni[1]{i},\pwlni[2]{i},\pnwlni[2]{i}) \in \dFs \times H_0^1(\dom{1})$ for each iterate of the \LDD solver, in order to obtain a solution to \autoref{problem:LDD-TPR:limitsystem:TPR:movingPhase} and thus \autoref{env:LDD-TPR:DiscontiuousProblemFormulation:TPR:semiDiscrete:weak}.
    One strength of the \LDD schemes presented in this thesis is precisely not to enforce the desired coupling condition in each iterate but only in the limit. 
    In view of this, the coupling conditions (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-wetting2}) and (\ref{eqn:LDD-TPR:MovingPhase.TPR.strong-nonwetting2}) seem a more desirable choice for enforcing moving phase conditions in the \TPR case.
\end{remark}


\begin{remark}[Open question: convergence]
Notice, that the proof of \autoref{LDD-TPR:convergence:theorem} does not carry over in a straight forward manner to the situation discussed here, because the functionals on the interface cannot be treated as in the proofs of Theorems \ref{LDD-TPR:convergence:theorem}, \ref{LDD-TPTP:mainresult} and \ref{LDD-RR:mainresult}. 
Notably, we do not get simple analoga to (\ref{eqn:LDD-TPR:gli:errors}), p. \pageref{eqn:LDD-TPR:gli:errors} and testing with the pressure errors does not lead to norms anymore. 

Thorough analysis and numerical testing of this proposition are questions for future work. 
Since the analysis of discontinuous capillary pressures in \cite{Cances2012} uses capillary pressures directly as primary unknowns it might be more promising to look for an \LDD formulation that makes use of capillary pressures as primary variables directly. 
\end{remark}


==> Sections/LDD-TwoPhaseRichards-main.tex <==
\section{Introduction} 
\input{Chapters/LDD-TwoPhaseRichards/LDD-TPR_introduction.tex}

\section{Problem description}
\label{LDD-TPR:section:problemFormulation}
\input{Chapters/LDD-TwoPhaseRichards/LDD-TPR_problem_formulation.tex}

\section{Convergence of the \ldd-\TPR solver}
\label{LDD-TPR:section:ConvergenceOfScheme}
\input{Chapters/LDD-TwoPhaseRichards/LDD-TPR_convergence.tex}
\section{Multi-domain formulation} 
\label{LDD-TPR:section:problemFormulation:multiDomain}
\input{Chapters/LDD-TwoPhaseRichards/LDD-TPR_multidomain_formulation.tex}
\section{Alternative coupling conditions} 
\label{LDD-TPR:section:AlternativeCouplingConditions}
\input{Chapters/LDD-TwoPhaseRichards/LDD-TPR_alternative_coupling_conditions.tex}

\section{Numerical validation of the \LDDTPR solver} 
\label{LDD-TPR:section:NumericalSection}
\input{Chapters/LDD-TwoPhaseRichards/LDD-TPR_numerical_section.tex}

\section{Conclusion}
\input{Chapters/LDD-TwoPhaseRichards/LDD-TPR_conclusion.tex}
\section*{Acknowledgements}

This chapter's work was supported by E.ON Stipendiensfonds and partly prepared at the University of Bergen 
(UIB) in collaboration with Prof. Florin A. Radu.


==> Tables/TPR2patchCoefficientsExactSolutionsTable.tex <==
\begin{tabular}{ l  l }
% \hline %&& \\ %to .49\textwidth {X[c,m] X[2.2,c,m] X[2.2,c,m] }%\hline%
    % initial condition
    %\taburowcolors[1]1{black!70 .. white}
    %\multicolumn{3}{c} {\textcolor{white}{\bf Boundary and Initial Conditions for Analytical Case}} \\
%   \rowfont\bfseries\textcolor{white}%
%   \rowcolor[gray]{0.75}
    %
    $\dom{1}$
        & $\dom{2}$	\\%\thkhline
    %
    %\taburowcolors[1]2{white .. gray!25}
    
    $\kwln[1]{}(s) = s^2$
    &$\kwln[2]{}(s) = s^3$	\\
    %
    
    \textcolor{gray}{$\knwln[1]{}(s) = (1-s)^2$}
    &$\knwln[2]{}(s) = (1-s)^3$	\\%[2ex]
    %
    $S_1(p_c) = \begin{cases}
        \frac{1}{(1 + p_c)^{1/2}} & p_c \geq 0 \\
        \hspace{7.25mm}1           & p_c < 0
        \end{cases} $
        & $S_2(p_c) = \begin{cases}
        \frac{1}{(1 + p_c)^{1/3}} & p_c \geq 0 \\
        \hspace{7.25mm}1          & p_c < 0
        \end{cases}$\\
%
$\pwln[1]{e}(x, y, t) =  -7 - \bigl(1+t^2\bigr)\bigl(1 + x^2 + y^2\bigr)$ 
        & $\pwln[2]{e}(x,y, t) = -7 - \bigl(1+t^2\bigr)\bigl(1 + x^2\bigr)$  \\%$ \pwln[2]{e}(x,y, t) = -5 - \bigl(1+t^2\bigr)\bigl(1 + x^2\bigr)$ \\
    % 
    -
        & $\pnwln[2]{e}(x,y, t) = \bigl(-1 -t(1.1 + y + x^2)\bigr)y^2$%\\[1em]
    % boundary condition
\end{tabular}


==> Tables/TPR2patchRealisticParameters.tex <==
%%% 
% \setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{1.3}
% \rowcolors{2}{white}{gray!25}
\begin{tabular}{ c c c c c} %m{5.6cm}  m{7.8cm} }
% \hline %&& \\ %to .49\textwidth {X[c,m] X[2.2,c,m] X[2.2,c,m] }%\hline%
  % initial condition
  %\taburowcolors[1]1{black!70 .. white}
  \multicolumn{5}{l}{\textcolor{black}{\scshape \TPR on two subdomain: Assumed soil parameters}} \\
%   \rowfont\bfseries\textcolor{white}%
  \rowcolor[gray]{0.75}  
%   \rowcolor[gray]{0.70}
  %
    \multicolumn{1}{r}{\scshape Parameter} & \multicolumn{2}{c}{\boldmath $\dom{1}$}
        & \multicolumn{2}{c}{\boldmath $\dom{2}$}	\\
    %
    $\Phi_l$& \multicolumn{2}{c}{0,22}
        & \multicolumn{2}{c}{0,0022}	\\
    %    
    $g[\si{\meter\per\square\second}]$ & \multicolumn{2}{c}{0}
        & \multicolumn{2}{c}{0}	\\
    %
    \rowcolor[gray]{0.85}  
%     \multicolumn{1}{r}{\bfseries Parameter}
        & {\bfseries wetting} & {\bfseries nonwetting} & {\bfseries wetting} & {\bfseries nonwetting} \\
%   %
  $\mu_{\alpha}[\si{\kilo\gram\per(\meter\second)}]$
    & 1 & - & 1 & $\frac{1}{50}$
      \\
  $\rho_{\alpha}[\si{\kilo\gram\per\cubic\meter}]$
    & 997 & - & 997 & 1,225 
      \\
%   %
%   $y=1$
%     &\rule{0pt}{2em}$\begin{aligned}
%        \pwln[1]{e}(x,1, t) &= -6 - \bigl(1+t^2\bigr)\bigl(2 + x^2\bigr) \\ 
%        \pnwln[1]{e}(x,1, t) &= -1 -2.1t
%      \end{aligned}$
%      \rule{0pt}{2em}
%       & - \\
%   $x=-1$
%     &\rule{0pt}{2em}$\begin{aligned}
%        \pwln[1]{e}(-1,y, t) &= -6 - \bigl(1+t^2\bigr)\bigl(2 + y^2\bigr) \\ 
%        \pnwln[1]{e}(-1,y, t) &= -1 -t\bigl(1.1+ y^2\bigr)
%      \end{aligned}$
%      \rule{0pt}{2em}
%       &	$\begin{aligned}
%        \pwln[2]{e}(-1,y, t) &= -6 - 2\bigl(1+t^2\bigr) \\ 
%        \pnwln[2]{e}(-1,y, t) &= -1 -t\bigl(1.1+ y^2\bigr) - \sin\bigl((-y-0.5t)y^2\bigr)^2
%      \end{aligned}$				\\
%   %
%   $x=1$
%     & \rule{0pt}{2em}$\begin{aligned}
%        \pwln[1]{e}(1,y, t) &= -6 - \bigl(1+t^2\bigr)\bigl(2 + y^2\bigr) \\ 
%        \pnwln[1]{e}(1,y, t) &= -1 -t\bigl(1.1+ y^2\bigr)
%      \end{aligned}$
%      \rule{0pt}{2em}
%       &
%       $\begin{aligned}
%        \pwln[2]{e}(1,y, t) &= -6 - 2\bigl(1+t^2\bigr) \\ 
%        \pnwln[2]{e}(1,y, t) &= -1 -t\bigl(1.1+ y^2\bigr) - \sin\bigl((y-0.5t)y^2\bigr)^2
%      \end{aligned}$	\\[1em]
\end{tabular}


==> Tables/TPRLayeredSoilDifferentIntrinsicVanGMualemCoefficientsExactSolutionsTable.tex <==
\begin{tabular}{c r c l r c l}
% \multicolumn{3}{l}{\scshape \tptp: Data and exact solutions}\\
% \toprule
%         & \Richards 
%             & two-phase \\
%     {\scshape Data}
       & & & $\dom{1}$, $\dom{2}$
            & & & $\dom{3}$, $\dom{4}$	\\[2ex]%\midrule
        & $\kwln{}(s)$ & $=$ & $\sqrt{s}\left[1-\bigl(1-s^{3/2}\bigr)^{2/3}\right]^2$
            & $\kwln{}(s)$ & $=$ &$\sqrt{s}\left[1-\bigl(1-s^{6/5}\bigr)^{5/6}\right]^2$	\\[2ex]
    %
        %
%     $\knwln{}(s)$
        &$\knwln{}(s)$ & $=$ & $(1-s)^{1/3}\left[1-s^{3/2}\right]^{4/3}$
            &$\knwln{}(s)$ & $=$ & $(1-s)^{1/3}\left[1-s^{6/5}\right]^{10/6}$	\\[2ex]
%     %
%     $S_l(p_c)$
        &
        $S_l(p_c)$ &$=$ & $\begin{cases}
            \frac{1}{(1 + (\num{0.001}p_c)^{3})^{2/3}} & p_c \geq 0 \\
            \hspace{7.25mm}1           & p_c < 0
        \end{cases} $
            & $S_l(p_c)$ &$=$ & $\begin{cases}
                \frac{1}{(1 + (\num{0.001}p_c)^{6})^{5/6}} & p_c \geq 0 \\
                \hspace{7.25mm}1          & p_c < 0
              \end{cases}$%\\ \addlinespace[0.75ex]
% \midrule
% %     {\scshape \makecell{Exact \\[-1ex] solution}}
% %         & $\dom{1}$
% %             & $\dom{2}$	\\\hline%\thkhline
% % 
%     $\pwln{e}(x, y, t)$
%         &$-7 - \bigl(1+t^2\bigr)\bigl(1 + x^2 + y^2\bigr)$ 
%             & $ -7 - \bigl(1+t^2\bigr)\bigl(1 + x^2\bigr)$ \\
%     % 
%     $\pnwln{e}(x,y, t)$
%         &  -
%             & $\bigl(-2-t(1.1+y + x^2)\bigr)y^2$\\
%     % boundary condition
%     \addlinespace[0.5ex]
%     \bottomrule
\end{tabular}


==> Tables/TPRLayeredSoilIPRealisticParametersDifferentIntrinsic.tex <==
\begin{tabular}{ c c c c c c c} %{0.65\textwidth}m{5.6cm}  m{7.8cm} }
%   \multicolumn{5}{l}{{\scshape \TPTP mesh study: Assumed soil parameters}} \\  
\toprule
        & \multicolumn{2}{c}{\Richards} 
            & \multicolumn{4}{c}{two-phase} \\
%
\multicolumn{1}{r}{\scshape Parameter} 
    & \multicolumn{2}{c}{$\dom{1}$, $\dom{2}$}
        & \multicolumn{2}{c}{$\dom{4}$} 
            & \multicolumn{2}{c}{$\dom{3}$, $\dom{5}$, $\dom{6}$}	\\\midrule
%
$\Phi_l$
    & \multicolumn{2}{c}{\num{0,57}}
        & \multicolumn{2}{c}{\num{0,005}} 
            & \multicolumn{2}{c}{\num{0,005}}	\\
%         
$k_{\mathsf{i},l}$
    & \multicolumn{2}{c}{\num{0,1}}
        & \multicolumn{2}{c}{\num{0,001}} 
            & \multicolumn{2}{c}{\num{0,001}}	\\
%    
% $g[\si{\meter\per\square\second}]$ & \multicolumn{2}{c}{\num{9.81}}
%     & \multicolumn{2}{c}{\num{9.81}}	\\
% %     
$h_{l}$
    & \multicolumn{2}{c}{\num{0.071}} 
        & \multicolumn{2}{c}{\num{0.070}} 
            & \multicolumn{2}{c}{\num{0.071}} \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
%
    $\alpha$ & $w$ & $\nw$ 
        & $w$ & $\nw$ 
            & $w$ & $\nw$ \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
%   %
$\mu_{\alpha}[\si{\kilo\gram\per(\meter\second)}]$
    & \num{1} & - 
        & \num{1} & $\frac{1}{50}$ 
            & \num{1} & $\frac{1}{50}$
    \\
$\rho_{\alpha}[\si{\kilo\gram\per\cubic\meter}]$
    & \num{997} & - 
        & \num{997} & \num{1,225} 
            & \num{997} & \num{1,225}  
    \\
% $L_{\alpha,l}$
%     & \num{0,5} & \num{0,25} & \num{0,5} & \num{0,25} \\
\bottomrule
\end{tabular}


==> Tables/TPRLayeredSoilIPRealisticParametersSameIntrinsic.tex <==
\begin{tabular}{ c c c c c c c} %{0.65\textwidth}m{5.6cm}  m{7.8cm} }
%   \multicolumn{5}{l}{{\scshape \TPTP mesh study: Assumed soil parameters}} \\  
\toprule
        & \multicolumn{2}{c}{\Richards} 
            & \multicolumn{4}{c}{two-phase} \\
%
\multicolumn{1}{r}{\scshape Parameter} 
    & \multicolumn{2}{c}{$\dom{1}$, $\dom{2}$}
        & \multicolumn{2}{c}{$\dom{4}$} 
            & \multicolumn{2}{c}{$\dom{3}$, $\dom{5}$, $\dom{6}$}	\\\midrule
%
$\Phi_l$
    & \multicolumn{2}{c}{\num{0,2}}
        & \multicolumn{2}{c}{\num{0,2}} 
            & \multicolumn{2}{c}{\num{0,2}}	\\
%         
$k_{\mathsf{i},l}$
    & \multicolumn{2}{c}{\num{0,01}}
        & \multicolumn{2}{c}{\num{0,01}} 
            & \multicolumn{2}{c}{\num{0,01}}	\\
%    
% $g[\si{\meter\per\square\second}]$ & \multicolumn{2}{c}{\num{9.81}}
%     & \multicolumn{2}{c}{\num{9.81}}	\\
% %     
$h_{l}$
    & \multicolumn{2}{c}{\num{0.071}} 
        & \multicolumn{2}{c}{\num{0.070}} 
            & \multicolumn{2}{c}{\num{0.071}} \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
%
    $\alpha$ & $w$ & $\nw$ 
        & $w$ & $\nw$ 
            & $w$ & $\nw$ \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
%   %
$\mu_{\alpha}[\si{\kilo\gram\per(\meter\second)}]$
    & \num{1} & - 
        & \num{1} & $\frac{1}{50}$ 
            & \num{1} & $\frac{1}{50}$
    \\
$\rho_{\alpha}[\si{\kilo\gram\per\cubic\meter}]$
    & \num{997} & - 
        & \num{997} & \num{1,225} 
            & \num{997} & \num{1,225}  
    \\
% $L_{\alpha,l}$
%     & \num{0,5} & \num{0,25} & \num{0,5} & \num{0,25} \\
\bottomrule
\end{tabular}


==> Tables/TPRLayeredSoilIPSameIntrinsicCoefficientsExactSolutionsTable.tex <==
\begin{tabular}{c  c  c}
% \multicolumn{3}{l}{\scshape \tptp: Data and exact solutions}\\
\toprule
        & \Richards 
            & two-phase \\
    {\scshape Data}
        &   $\dom{1}$, $\dom{2}$
            &  $\dom{3}$-$\dom{6}$	\\\midrule
    $\kwln{}(s)$
        & $s^2$
            & $s^3$	\\
    %
    $\knwln{}(s)$
        &$(1-s)^2$
            &$(1-s)^3$	\\%[2ex]
    %
    $S_l(p_c)$
        &
        $\begin{cases}
            \frac{1}{(1 + p_c)^{1/2}} & p_c \geq 0 \\
            \hspace{7.25mm}1           & p_c < 0
        \end{cases} $
            & $\begin{cases}
                \frac{1}{(1 + p_c)^{1/3}} & p_c \geq 0 \\
                \hspace{7.25mm}1          & p_c < 0
              \end{cases}$\\ \addlinespace[0.75ex]
\midrule
%     {\scshape \makecell{Exact \\[-1ex] solution}}
%         &  $\dom{1}$
%             & $\dom{2}$	\\\hline%\thkhline
% 
    $\pwln{e}(x, y, t)$
        &$-7 - \bigl(1+t^2\bigr)\bigl(1 + x^2 + y^2\bigr)$ 
            & $ -7 - \bigl(1+t^2\bigr)\bigl(1 + x^2\bigr)$ \\
    % 
    $\pnwln{e}(x,y, t)$
        &  -
            & $\bigl(-3-t(1+y + x^2) - t^2\bigr)y^2$\\
    % boundary condition
    \addlinespace[0.5ex]
    \bottomrule
\end{tabular}


==> Tables/TPRLayeredSoilRealisticParametersDifferentIntrinsicVanGMualem.tex <==
\xdef\hOne{0.071}
\xdef\hTwo{0.071}
\xdef\hThree{0.070}
\xdef\hFour{0.071}
\begin{tabular}{ c c c c c  c c c c } %m{5.6cm}  m{7.8cm} }
%   \multicolumn{5}{l}{{\scshape \TPTP mesh study: Assumed soil parameters}} \\  
  \toprule
  %
    \multicolumn{1}{r}{Parameter} & \multicolumn{2}{c}{$\dom{1}$}
        & \multicolumn{2}{c}{$\dom{2}$}	& \multicolumn{2}{c}{$\dom{3}$}
        & \multicolumn{2}{c}{$\dom{4}$}	\\\midrule
    %
    $\Phi_l$& \multicolumn{2}{c}{\num{0,37}}
        & \multicolumn{2}{c}{\num{0,22}} & \multicolumn{2}{c}{\num{0,02}} & \multicolumn{2}{c}{\num{0,022}}	\\
%         
    $k_{\mathsf{i},l}$& \multicolumn{2}{c}{\num{0.01}}
        & \multicolumn{2}{c}{\num{0.01}} & \multicolumn{2}{c}{\num{0.001}}
        & \multicolumn{2}{c}{\num{0.001}}	\\
    %    
    $g[\si{\meter\per\square\second}]$ & \multicolumn{2}{c}{\num{9.81}}
        & \multicolumn{2}{c}{\num{9.81}} & \multicolumn{2}{c}{\num{9.81}}
        & \multicolumn{2}{c}{\num{9.81}}	\\
%     
    $h_{l}$
        & \multicolumn{2}{c}{\hOne} & \multicolumn{2}{c}{\hTwo} & \multicolumn{2}{c}{\hThree} & \multicolumn{2}{c}{\hFour} \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}
    %
    $\alpha$ & $w$ & $\nw$ & $w$ & $\nw$ & $w$ & $\nw$ & $w$ & $\nw$ \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}
  %
    $\mu_{\alpha}[\si{\kilo\gram\per(\meter\second)}]$
        & \num{1} & $\frac{1}{50}$ & \num{1} & $\frac{1}{50}$ & \num{1} & $\frac{1}{50}$ & \num{1} & $\frac{1}{50}$
        \\
    $\rho_{\alpha}[\si{\kilo\gram\per\cubic\meter}]$
        & \num{997} & \num{1,225} & \num{997} & \num{1,225} & \num{997} & \num{1,225} & \num{997} & \num{1,225}  
      \\
    $L_{\alpha,l}$
        & \num{0,0025} & - & \num{0,0025} & - & \num{0,0025} & \num{0,0025} & \num{0,0025} & \num{0,0025} \\
    \bottomrule
\end{tabular}


% \begin{tabular}{ c c c c c} %{0.65\textwidth}m{5.6cm}  m{7.8cm} }
% %   \multicolumn{5}{l}{{\scshape \TPTP mesh study: Assumed soil parameters}} \\  
% \toprule
%         & \multicolumn{2}{c}{\Richards} 
%             & \multicolumn{2}{c}{two-phase} \\
% %
% \multicolumn{1}{r}{\scshape Parameter} 
%     & \multicolumn{2}{c}{$\dom{1}$, $\dom{2}$}
%         & \multicolumn{2}{c}{$\dom{3}$, $\dom{4}$}	\\\midrule
% %
% $\Phi_l$
%     & \multicolumn{2}{c}{\num{0,37}, \num{0,22}}
%           & \multicolumn{2}{c}{\num{0,2}, \num{0,22}}	\\
% %         
% $k_{\mathsf{i},l}$
%     & \multicolumn{2}{c}{\num{0,01}}
%             & \multicolumn{2}{c}{\num{0,01}}	\\
% %    
% % $g[\si{\meter\per\square\second}]$ & \multicolumn{2}{c}{\num{9.81}}
% %     & \multicolumn{2}{c}{\num{9.81}}	\\
% % %     
% $h_{l}$
%     & \multicolumn{2}{c}{\num{0.071}} 
%             & \multicolumn{2}{c}{\num{0.071}} \\        %\midrule
% %
%     & $w$ & $\nw$ 
%             & $w$ & $\nw$ \\
% %   %
% $\mu_{\alpha}[\si{\kilo\gram\per(\meter\second)}]$
%     & \num{1} & - 
%             & \num{1} & $\frac{1}{50}$
%     \\
% $\rho_{\alpha}[\si{\kilo\gram\per\cubic\meter}]$
%     & \num{997} & - 
%             & \num{997} & \num{1,225}  
%     \\
% % $L_{\alpha,l}$
% %     & \num{0,5} & \num{0,25} & \num{0,5} & \num{0,25} \\
% \bottomrule
% \end{tabular}


==> Tables/TPRLayeredSoilRealisticParametersSameIntrinsic.tex <==
\begin{tabular}{ c c c c c} %{0.65\textwidth}m{5.6cm}  m{7.8cm} }
%   \multicolumn{5}{l}{{\scshape \TPTP mesh study: Assumed soil parameters}} \\  
\toprule
        & \multicolumn{2}{c}{\Richards} 
            & \multicolumn{2}{c}{two-phase} \\
%
\multicolumn{1}{r}{\scshape Parameter} 
    & \multicolumn{2}{c}{$\dom{1}$, $\dom{2}$}
        & \multicolumn{2}{c}{$\dom{3}$, $\dom{4}$}	\\\midrule
%
$\Phi_l$
    & \multicolumn{2}{c}{\num{0,37}, \num{0,22}}
          & \multicolumn{2}{c}{\num{0,2}, \num{0,22}}	\\
%         
$k_{\mathsf{i},l}$
    & \multicolumn{2}{c}{\num{0,01}}
            & \multicolumn{2}{c}{\num{0,01}}	\\
%    
% $g[\si{\meter\per\square\second}]$ & \multicolumn{2}{c}{\num{9.81}}
%     & \multicolumn{2}{c}{\num{9.81}}	\\
% %     
$h_{l}$
    & \multicolumn{2}{c}{\num{0.071}} 
            & \multicolumn{2}{c}{\num{0.071}} \\        %\midrule
%
    & $w$ & $\nw$ 
            & $w$ & $\nw$ \\
%   %
$\mu_{\alpha}[\si{\kilo\gram\per(\meter\second)}]$
    & \num{1} & - 
            & \num{1} & $\frac{1}{50}$
    \\
$\rho_{\alpha}[\si{\kilo\gram\per\cubic\meter}]$
    & \num{997} & - 
            & \num{997} & \num{1,225}  
    \\
% $L_{\alpha,l}$
%     & \num{0,5} & \num{0,25} & \num{0,5} & \num{0,25} \\
\bottomrule
\end{tabular}


==> Tables/TPRLayeredSoilRealisticParametersSameIntrinsicVanGMualem.tex <==
\xdef\hOne{0.071}
\xdef\hTwo{0.071}
\xdef\hThree{0.070}
\xdef\hFour{0.071}
\begin{tabular}{ c c c c c  c c c c } %m{5.6cm}  m{7.8cm} }
%   \multicolumn{5}{l}{{\scshape \TPTP mesh study: Assumed soil parameters}} \\  
  \toprule
  %
    \multicolumn{1}{r}{Parameter} & \multicolumn{2}{c}{$\dom{1}$}
        & \multicolumn{2}{c}{$\dom{2}$}	& \multicolumn{2}{c}{$\dom{3}$}
        & \multicolumn{2}{c}{$\dom{4}$}	\\\midrule
    %
    $\Phi_l$& \multicolumn{2}{c}{\num{0,37}}
        & \multicolumn{2}{c}{\num{0,22}} & \multicolumn{2}{c}{\num{0,2}} & \multicolumn{2}{c}{\num{0,22}}	\\
%         
    $k_{\mathsf{i},l}$& \multicolumn{2}{c}{\num{0.01}}
        & \multicolumn{2}{c}{\num{0.01}} & \multicolumn{2}{c}{\num{0.01}}
        & \multicolumn{2}{c}{\num{0.01}}	\\
    %    
    $g[\si{\meter\per\square\second}]$ & \multicolumn{2}{c}{\num{9.81}}
        & \multicolumn{2}{c}{\num{9.81}} & \multicolumn{2}{c}{\num{9.81}}
        & \multicolumn{2}{c}{\num{9.81}}	\\
%     
    $h_{l}$
        & \multicolumn{2}{c}{\hOne} & \multicolumn{2}{c}{\hTwo} & \multicolumn{2}{c}{\hThree} & \multicolumn{2}{c}{\hFour} \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}
    %
   $\alpha$ & $w$ & $\nw$ & $w$ & $\nw$ & $w$ & $\nw$ & $w$ & $\nw$ \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}
  %
    $\mu_{\alpha}[\si{\kilo\gram\per(\meter\second)}]$
        & \num{1} & $\frac{1}{50}$ & \num{1} & $\frac{1}{50}$ & \num{1} & $\frac{1}{50}$ & \num{1} & $\frac{1}{50}$
        \\
    $\rho_{\alpha}[\si{\kilo\gram\per\cubic\meter}]$
        & \num{997} & \num{1,225} & \num{997} & \num{1,225} & \num{997} & \num{1,225} & \num{997} & \num{1,225}  
      \\
    $L_{\alpha,l}$
        & \num{0,1} & - & \num{0,9} & - & \num{0,9} & \num{0,025} & \num{0,08} & \num{0,025} \\
    \bottomrule
\end{tabular}


% \begin{tabular}{ c c c c c} %{0.65\textwidth}m{5.6cm}  m{7.8cm} }
% %   \multicolumn{5}{l}{{\scshape \TPTP mesh study: Assumed soil parameters}} \\  
% \toprule
%         & \multicolumn{2}{c}{\Richards} 
%             & \multicolumn{2}{c}{two-phase} \\
% %
% \multicolumn{1}{r}{\scshape Parameter} 
%     & \multicolumn{2}{c}{$\dom{1}$, $\dom{2}$}
%         & \multicolumn{2}{c}{$\dom{3}$, $\dom{4}$}	\\\midrule
% %
% $\Phi_l$
%     & \multicolumn{2}{c}{\num{0,37}, \num{0,22}}
%           & \multicolumn{2}{c}{\num{0,2}, \num{0,22}}	\\
% %         
% $k_{\mathsf{i},l}$
%     & \multicolumn{2}{c}{\num{0,01}}
%             & \multicolumn{2}{c}{\num{0,01}}	\\
% %    
% % $g[\si{\meter\per\square\second}]$ & \multicolumn{2}{c}{\num{9.81}}
% %     & \multicolumn{2}{c}{\num{9.81}}	\\
% % %     
% $h_{l}$
%     & \multicolumn{2}{c}{\num{0.071}} 
%             & \multicolumn{2}{c}{\num{0.071}} \\        %\midrule
% %
%     & $w$ & $\nw$ 
%             & $w$ & $\nw$ \\
% %   %
% $\mu_{\alpha}[\si{\kilo\gram\per(\meter\second)}]$
%     & \num{1} & - 
%             & \num{1} & $\frac{1}{50}$
%     \\
% $\rho_{\alpha}[\si{\kilo\gram\per\cubic\meter}]$
%     & \num{997} & - 
%             & \num{997} & \num{1,225}  
%     \\
% % $L_{\alpha,l}$
% %     & \num{0,5} & \num{0,25} & \num{0,5} & \num{0,25} \\
% \bottomrule
% \end{tabular}


==> Tables/TPRLayeredSoilSameIntrinsicCoefficientsExactSolutionsTable.tex <==
\begin{tabular}{c  c  c}
% \multicolumn{3}{l}{\scshape \tptp: Data and exact solutions}\\
\toprule
        & \Richards 
            & two-phase \\
    {\scshape Data}
        &  $\dom{1}$, $\dom{2}$
            &  $\dom{3}$,$\dom{4}$	\\\midrule
    $\kwln{}(s)$
        & $s^2$
            & $s^3$	\\
    %
    $\knwln{}(s)$
        &$(1-s)^2$
            &$(1-s)^3$	\\%[2ex]
    %
    $S_l(p_c)$
        &
        $\begin{cases}
            \frac{1}{(1 + (\num{0.001}p_c)^{3})^{2/3}} & p_c \geq 0 \\
            \hspace{7.25mm}1           & p_c < 0
        \end{cases} $
            & $\begin{cases}
                \frac{1}{(1 + (\num{0.001}p_c)^{6})^{5/6}} & p_c \geq 0 \\
                \hspace{7.25mm}1          & p_c < 0
              \end{cases}$\\ \addlinespace[0.75ex]
\midrule
%     {\scshape \makecell{Exact \\[-1ex] solution}}
%         & $\dom{1}$
%             & $\dom{2}$	\\\hline%\thkhline
% 
    $\pwln{e}(x, y, t)$
        &$-6 - \bigl(1+t^2\bigr)\bigl(1 + x^2 + y^2\bigr)$ 
            & $ -6 - \bigl(1+t^2\bigr)\bigl(1 + x^2\bigr)$ \\
    % 
    $\pnwln{e}(x,y, t)$
        &  -
            & $\bigl(-1-t(1.1+y + x^2)\bigr)y^2$\\
    % boundary condition
    \addlinespace[0.5ex]
    \bottomrule
\end{tabular}


==> Tables/TPRLayeredSoilSameIntrinsicVanGMualemCoefficientsExactSolutionsTable.tex <==
\begin{tabular}{c  c  c}
% \multicolumn{3}{l}{\scshape \tptp: Data and exact solutions}\\
\toprule
        & \Richards 
            & two-phase \\
    {\scshape Data}
        &  $\dom{1}$, $\dom{2}$
            &  $\dom{3}$,$\dom{4}$	\\\midrule
    $\kwln{}(s)$ 
        & $\sqrt{s}\left[1-\bigl(1-s^{3/2}\bigr)^{2/3}\right]^2$
            & $\sqrt{s}\left[1-\bigl(1-s^{5/4}\bigr)^{4/5}\right]^2$	\\[1ex]
    %
        %
    $\knwln{}(s)$
        &$(1-s)^{1/3}\left[1-s^{3/2}\right]^{4/3}$
            &$(1-s)^{1/3}\left[1-s^{5/4}\right]^{8/5}$	\\[1ex]
    %
    $S_l(p_c)$
        &
        $\begin{cases}
            \frac{1}{(1 + (\num{0.001}p_c)^{3})^{2/3}} & p_c \geq 0 \\
            \hspace{7.25mm}1           & p_c < 0
        \end{cases} $
            & $\begin{cases}
                \frac{1}{(1 + (\num{0.001}p_c)^{5})^{4/5}} & p_c \geq 0 \\
                \hspace{7.25mm}1          & p_c < 0
              \end{cases}$\\ \addlinespace[0.75ex]
\midrule
%     {\scshape \makecell{Exact \\[-1ex] solution}}
%         & $\dom{1}$
%             & $\dom{2}$	\\\hline%\thkhline
% 
    $\pwln{e}(x, y, t)$
        &$-7 - \bigl(1+t^2\bigr)\bigl(1 + x^2 + y^2\bigr)$ 
            & $ -7 - \bigl(1+t^2\bigr)\bigl(1 + x^2\bigr)$ \\
    % 
    $\pnwln{e}(x,y, t)$
        &  -
            & $\bigl(-2-t(1.1+y + x^2)\bigr)y^2$\\
    % boundary condition
    \addlinespace[0.5ex]
    \bottomrule
\end{tabular}

